Personalized Federated Learning of Driver Prediction Models for Autonomous Driving

Autonomous vehicles (AVs) must interact with a diverse set of human drivers in heterogeneous geographic areas. Ideally, fleets of AVs should share trajectory data to continually re-train and improve trajectory forecasting models from collective experience using cloud-based distributed learning. At the same time, these robots should ideally avoid uploading raw driver interaction data in order to protect proprietary policies (when sharing insights with other companies) or protect driver privacy from insurance companies. Federated learning (FL) is a popular mechanism to learn models in cloud servers from diverse users without divulging private local data. However, FL is often not robust -- it learns sub-optimal models when user data comes from highly heterogeneous distributions, which is a key hallmark of human-robot interactions. In this paper, we present a novel variant of personalized FL to specialize robust robot learning models to diverse user distributions. Our algorithm outperforms standard FL benchmarks by up to 2x in real user studies that we conducted where human-operated vehicles must gracefully merge lanes with simulated AVs in the standard CARLA and CARLO AV simulators.

==> figure_latex/lane_change.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=1.0\columnwidth]{pics/lane_change.pdf}
    \caption{\small{\textbf{The lane change scenario}:
    The blue car (lower left) driven by a human is going to change the lane while considering relative position ,velocity  to other vehicles and driver's own driving style.
    The red car (upper row) is a robot driving car that predicts human driving car’s control and trying to the entire traffic smooth and safe.
    The green car (lower right) is always going straight but sometimes a obstacle to the blue car.}}
    \label{fig:lane_change_scenario}
\vspace{-1em}
\end{figure}


==> figure_latex/lane_swapping.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=1.0\columnwidth]{pics/lane_swapping.pdf}
    \caption{\small{\textbf{The lane swapping scenario}:
    A couple of cars have to change lanes in the limited distance while keeping safe distance from another vehicle. The blue car (bottom row) is a human driving car that has an individual driving style, and the red car (upper row) is a robot driving car that predicts human driving car’s control.}}
    \label{fig:lane_swapping_scenario}
\vspace{-1em}
\end{figure}


==> sections/backup/experiments.tex <==
\input{figure_latex/LQR_system.tex}

We evaluate the proposed method through three different tasks.
The first one is a very simple task to see how the proposed method fundamentally works.
The second and third are more practical tasks about autonomous driving where a robot vehicle changes a lane while taking into consideration the behavior of other vehicles including human's vehicles.

\subsection{LQR control of 1-dimension mass point}
\label{subsec:LQR_eval}

\begin{comment}
\begin{enumerate}
    \item motivate why we introduce such a simple task.
    \item explain the system (state, action etc..) and control policy
    \item explain how we collect the dataset for training.
    \item describe training methods and evaluation metrics
    \item show results: One-fits-all methods are good at learning dynamics but not at learning individual preferences. Local training that uses only a single type of data is able to learn individual preference but takes a long time to converge. PFL is not only able to learn common dynamics but individual preferences.
\end{enumerate}
\end{comment}

In this section, we introduce a very simple task dealing with the motion of a mass point controlled with the linear-quadratic regulator (LQR) in the 1-dimension space.
The robots aim to move a mass point to the specific position from an arbitrary initial position with LQR controller.
The evaluation of this task, whose dynamics is completely known, enables us to see how well the proposed method works.

In this task, $x^t_k$ in Sec. \ref{sec:proposed_method}, which is the whole system state measured by $\mathcal{R}_k$ at time $t$,
can be denoted by $(v_t, y_t)^\mathrm{T}$ in illustrated in Fig. \ref{fig:LQR_1d_system}.
This simple system can be described with a linear system, and the system state equation of a linear system is generally defined as $x^{t+1}_k = Ax^t_k + Bu^t_k$, where $A$ and $B$ are coefficient matrices ($A \in \mathbb{R}^{i \times i}, B \in \mathbb{R}^{i \times j} ; i,j \in \mathbb{N}$) and $u^t_k$ is control input. In particular, $u^t_k$ of this system is denoted by 1-dimension vector $(u_t)$. 
Therefore, the state equation of this system is as follows.
\begin{small}
\begin{align*}
\begin{pmatrix}v_{t+1} \\ y_{t+1}\end{pmatrix} = A\begin{pmatrix}v_t\\y_t\end{pmatrix} + B\begin{pmatrix}u_t\end{pmatrix}
\end{align*}
\end{small}
Furthermore, the relation $v_{t+1} = v_t + u_t$ and  $y_{t+1} = y_t + v_t$ holds because of the equation of motion, $u = dv/dt$ (mass $m=1$ for simplicity).
Putting these equations together, the state equation above is converted as follows.
\begin{small}
\begin{align*}
x^{t+1}_k = \begin{pmatrix}1 & 1 \\0 & 1\end{pmatrix}x^t_k + \begin{pmatrix}0\\1\end{pmatrix} u^t_k
\end{align*}
\end{small}
Next, we define a cost function to identify the optimal control input.
The cost function of the LQR controller is defined as $\sum_{t=0}^{\infty} (x^\mathrm{T} Q x + u^\mathrm{T} R u)$, where $Q$ and $R$ are weight matrices ( $Q \in \mathbb{R}^{i \times i}, R \in \mathbb{R}^{j \times j}$ ).
In general, the optimal control input $u^*_t$ is known as $-Kx^{t-1}_k$ where $K = R^{-1}B^{T}P$, and $P \in \mathbb{R}^{i \times i}$ is the solution to the following Riccati equation:
\begin{small}
\begin{align*}
PA+A^\mathrm{T}P-PBR^{-1}B^\mathrm{T}P+Q=0
\end{align*}
\end{small}
In this experiment, we assume that $\mathcal{R}_k$ knows the construction of the system state equations above but does not know its parameters such as $A$, $B$, $Q$ and $R$,
and $\mathcal{R}_k$ try to estimate these parameters from the set of the measured trajectory data to predict the system state and optimal control input.
we note that it is enough to estimate parameter matrices $A$, $B$ and $K$ to predict them
because all $\mathcal{R}_k$ should know to predict next state are knowledge about the system state equation, the value of $x^t_k$, $A$, $B$, and $K$.

What we want to emphasize in this experiment is $A$ and $B$ should converge to the same value on any training dataset
since the only rule the system state follows is the equation of motion that does not depend on any control preference.
Using this knowledge about the parameters, we can validate our hypothesis that the parameters independent of $\mathcal{R}_k$ should not be trained in the personalized training.

\noindent \tu{Dataset:}
We generated three types of synthetic dataset from the system state equation and different cost functions.
They are different in how much rapid control is allowed.
We fixed the weight matrix $Q$ as an identity matrix but varied $R$ for simplicity.
The first is the reference controller whose $R$ is 1.
The second and Third are 50 and 100, respectively.
The larger $R$, the more rapid control is allowed.
During simulation, we added noise to system state and control input, which follows a Gaussian distribution with little variance.
Using the controllers obtained by these cost functions, we collected the trajectories of a mass point which starts with randomly initialized $x^0_k$.
The number of initial states is 40 and we executed a simulation for 30 time steps ($T=30$) in every simulation. Therefore, the number of total states collected is $3,600 (40 \times 30 \times 3)$. 10\% of the data is used only for evaluation of test loss, which is one of the evaluation metrics.

\noindent \tu{Benchmark Algorithms:}
To compare to the proposed method, we evaluated five algorithms shown in Tab. \ref{tab:algorithms}.
We used FedAVG to aggregate the parameters trained on each robot.
In the methods that hold personalized training on the robots, we assume that each robot observes only one type of data.
Therefore, there are three robots and they connect to a cloud environment for exchange of learned parameters.

As mentioned in Tab. \ref{tab:algorithms}, adaptive pesronalized FL (APFL) of this experiments do not adjust learning rate as we showed in Sec. \ref{sec:proposed_method} because the parameter to be trained in personalized training is obviously $K$.
Therefore, APFL only trains $K$ in personalized training, and we see if our method is essentially effective.

\begin{table}[t]
\caption{{\textbf{Description of training algorithms}}}
\label{tab:algorithms}
\centering
\begin{tabular}{p{2.7cm}|p{5cm}}
    \hline
    Name & Description \\
    \hline \hline
    Local & All robots train their models only on the data measured from themselves. \\ \hline
    Cloud & Training is processed on the cloud environment using all data. \\ \hline
    Standard FL (SFL) & The standard federated learning which is the same as Alg. \ref{alg:train} except there is no personalization part (line 7). \\ \hline
    Standard Personalized FL (SPFL) & The standard personalized FL which is Alg. \ref{alg:train} without applying parameter-wise learning rate \\ \hline
    Adaptive Personalized FL (APFL) & The proposed method itself shown in Alg. \ref{alg:train}. In case of the experiment in \ref{subsec:LQR_eval}, instead of applying parameter-wise learning rate, only the parameter $K$ is trained during the personalized training. This is the same as applying the ideal learning rate. \\ \hline
\end{tabular}
\end{table}

\noindent \tu{Evaluation Metrics:}
We evaluated the prediction losses for the test data and divergence of the learned parameters from true parameters ($A$,$B$ and $K$) because true parameters are known in this experiment.
We use the mean squared error (MSE) as the prediction loss, which corresponds to the objective function in Sec. \ref{sec:proposed_method}.
Therefore, the loss function $F(\mathbf{x}_k;\theta_k)$ is denoted by $1/|\mathbf{x}_k|\sum_{k,t}((\hat{x^t_k}-x^t_k)^2+(\hat{u^t_k}-u^t_k)^2)$ where $\hat{x^t_k}$ and $\hat{u^t_k}$ are prediction vectors of system state and control input computed by $\hat{A}x^{t-1}_k + \hat{B}u^{t-1}_k$ and $-\hat{K}x^{t-1}_k$, respectively.

The methods generate multiple personalized models such as Local, Standard Personalized FL and Adaptive Personalized FL are evaluated with average of prediction loss for all three models.
Personalized models are evaluated with only one type of test data corresponding to that of training data.
The optimization method we used is ADAM \cite{kingma2014adam}, and both the default learning rate and $L$ are 0.01.

\begin{table}[t]
\caption{\small{\textbf{Prediction loss for each algorithm}:
The theoretical lower bound of the prediction loss is 0.01 due to the gaussian noise added to the measured system state and control.
All the losses are mean of 10 trials.
}}
\label{tab:LQRloss}
\centering
\begin{tabular}{c|c|c|c|c|c}
    \hline
    Algorithm & Local & Cloud & SFL & SPFL & APFL \\ \hline
    \hline
    State Loss & 0.01101 & \textbf{0.01012} & 0.01023 & 0.01023 & 0.01020 \\ \hline
    Control Loss & 0.01251 & 0.19666 & 0.20123 & \textbf{0.01095} & 0.01096 \\ \hline
    Total Loss & 0.02352 & 0.20678 & 0.21146 & 0.02118 & \textbf{0.02116} \\ \hline
\end{tabular}
\end{table}

\input{figure_latex/LQR_distance.tex}

\noindent \tu{Results:}
Tab. \ref{tab:LQRloss} shows the prediction losses for each training method.
We show the prediction loss of system state ($x^t_k$ predicted by $A$ and $B$) and control ($u^t_k$ predicted by $K$) separately to see how differently learned the common parameters and customized for each data type.
The most methods including federated learning are able to learn the state dynamics, which is a common parameter.
However, Local is the worst loss due to little amount of training data.
In terms of the control loss, the methods with personalization (Local, SPFL and APFL) outperforms others that train one-size-fits-all model only.
APFL has the lowest total loss but the difference from SPFL is very small.

Fig. \ref{fig:LQR_distance} shows how close the learned parameters converged to the true parameters.
We can much clearly see effectiveness of not only FL algorithms with personalization but also selection of the parameter to be trained.
This implies our method should work well in learning of more complicated model.
In the next two evaluation cases, we make sure if that is correct.

\subsection{Lane swapping with light-weight simulator}
\label{subsec:lane_swapping}

\begin{comment}
\begin{enumerate}
    \item discuss CARLO and how its a light-weight simulator
    \item motivate why lane swapping is a good example to test different human driving styles, cite the Schmerling ICRA 2018 paper
    \item describe how we set up experiments: cost function, robot vehicle cost function, and how many users/trials we gathered data for
    \item show a figure of CVAE and describe the model architecture
    \item show the learning curve showing how personalized federated converges better and describe the boxplots quantitatively
\end{enumerate}
\end{comment}

The second case is a simulation of a practical driving scenario shown on the left side of Fig. \ref{fig:traffic_scenarios}.
The objective of this experiment is to see how the proposed algorithm works in such a scenario with a dataset generated by real humans.
The lane swapping scenario was used for a prediction model of human driving \cite{schmerling2018multimodal}, and is also a good example to test different human driving styles because we expect that datasets observed by robots are very different depending on a human driving style.
For example, a robot will observe the human car aggressively accelerating if the human driver tends to pass other cars to changing a lane.
Thus, trajectories of human cars show their driving preferences since a driver must choose to pass or let another car go to change a lane.

We used CARLO \cite{cao2020reinforcement}, which is a light-weight 2D driving simulator, as the simulation environment
because it is easy to run the scenario and collect datasets of real human driving on ordinary computers that does not equip powerful GPUs and a special human interface.

%\input{figure_latex/lane_swapping.tex}
\input{figure_latex/traffic_scenarios.tex}

\noindent \tu{System Definition:}
We define the system state $S_t$ as $(\vec{p}^{\;r}_t, \vec{p}^{\;h}_t, \vec{v}^{\;r}_t, \vec{v}^{\;h}_t)$ where $\vec{p}^{\;r}_t$ and $\vec{p}^{\;h}_t$ are the 2D position vectors of the robot and human car at discrete time $t$, and $\vec{v}^{\;r}_t$ and $\vec{v}^{\;r}_t$ are the velocity vectors.
The 2D vectors are decomposed into $x$ and $y$ components.
For example, a robot's velocity is denoted by $\vec{v}^{\;r}_t = (v^{rx}_t, v^{ry}_t)$ where $v^{rx}_t$ and $v^{ry}_t$ are scalar values representing a robot's velocity of lateral and longitudinal direction.

The control space of cars involves throttle and steering
which are finite sets represented as $\{-1.5,0,1.5\}$ and $\{-0.04,0,0.04\}$, respectively.
For example, the throttle of a robot is denoted by $c^{rth}_t \in \{-1.5,0,1.5\}$.
Similarly, the steering of a human is denoted by $c^{hst}_t \in \{-0.04,0,0.04\}$.
Thus, the control of the cars at time $t$ is denoted by $C_t = (C^r_t, C^h_t) = (c^{rth}_t, c^{rst}_t, c^{hth}_t, c^{hst}_t)$.

\noindent \tu{Prediction Model:}
%Description of CVAE
The robot controller has to make prediction of future system states to choose the proper control inputs.
In this experiment,
we assume that robots can measure current system state and control,
and know the system dynamics such as physical law.
Under the such assumption, all robots need to predict is human's control inputs.
This is because that robots are able to compute future system states sequentially from the current state and future controls.
Additionally, we take the prediction sequence used in Model Predictive Control (MPC) \cite{MPC}, which is widely used for modern control problems.
Specifically, we assume robot control inputs are periodically decided with the interval $\tau$.
This means that the prediction model need to estimate a series of human control inputs at a single prediction.
To achieve this, we introduce a Conditional Variational Autoencoder (CVAE) illustrated in Fig. \ref{fig:cvae_arch} with recurrent subcomponents \cite{schmerling2018multimodal} which is able to predict time-series data.

\noindent \tu{Robot Controller:}
%Cost function, policy etc..
We define the robot controller as a two-phase controller.
In the first phase, the controller is responsible for negotiating the longitudinal distance between human vehicles with different driving styles.
This is the most important part in our experiment because it is a part where we can see controller performance in terms of personalization.
For the first phase, we introduce a cost function $J_t$ to evaluate control inputs candidates at time $t$ as the following.
\begin{small}
\begin{align*}
    J_t = \alpha (p^{ry}_{t} - p^{hy}_{t}) (v^{ry}_{t} - v^{hy}_{t}) + \beta / |\vec{p}^{\;r}_{t} - \vec{p}^{\;h}_{t}|
\end{align*}
\end{small}
The first term represents longitudinal cost based on the fact that cars need sufficient longitudinal distance during lane change.
The second term represents distance cost to avoid collision.
$\alpha$ and $\beta$ are parameters to be manually tuned. We decided that they are $-3$ and $5000$ in this experiment.

When the robot controller decides a series of control inputs $[(c^{rth}_{t+1}, c^{rst}_{t+1}), (c^{rth}_{t+2}, c^{rst}_{t+2}),..,(c^{rth}_{t+\tau}, c^{rst}_{t+\tau})]$ at time $t$,
a robot computes the sum of the expected cost function in the time horizon $H>\tau$ for all robot control candidates.
To the end, a robot controller choose a series of control inputs that minimizes the sum of the expected cost function.
We set $\tau$ and $H$ to $3$ and $20$ due to computational limitation.

Once there is the enough longitudinal distance to swap lanes, the controller switches to the second phase, and just working as a lane change controller.
Since human's driving styles almost do not differ in the lane change,
we implemented it with a static LQR controller so that a robot car can get a target lateral position $p^{rx}$ representing x-coordinate of a target lane and longitudinal velocity $v^{ry}$ for simplicity.

In the evaluation, we incorporate the prediction model trained with some different ways into the robot controller,
and compare these controllers in terms of how safe and efficiently the cars are able to swap lanes under the different human's driving styles.

\input{figure_latex/cvae_arch.tex}

\noindent \tu{Dataset:}
The dataset of this experiment is a set of session data which have all the system states from time $0$ to the time when the both cars finished to run the specified distance.
There are two types of the dataset in this experiment.
First is for training of the prediction model. The another one is for evaluation.
In order to add diversity to each session data, we randomly created 50 initial states $S_0$.

For the first dataset, seven humans play the lane swapping scenario running on the CARLO simulator with 50 initial states above.
Since the prediction model with CVAE shown in Fig. \ref{fig:cvae_arch} is not trained at this time,
the robot controller use a very simple model based on the only current state.
Specifically, the predicted human control $\hat{C}^h_i$ for future time $i$ is always the current human control $C^h_t$ for any $i \in \{t+1,t+2,..,t+\tau\}$.

The second dataset, which is for evaluation, is basically generated with the same process of the first dataset
but the prediction model used in the robot controller is trained on the first dataset.
Similar to the experiment \ref{subsec:LQR_eval}, each robot car observes the only one type of data corresponding to one human driver.
Therefore, there are seven robots in the system.
During training, both the default learning rate and $L$ are 0.001, and the loss function is evidence lower bound objective (ELBO) \cite{kingma2013auto,rezende2014stochastic}.
The number of epochs is 30 for each training step in Alg. \ref{alg:train}.
We used 40 sessions for training and the rest 10 sessions for testing when we train the prediction model.
We trained the model with four algorithms except Local shown in Tab. \ref{tab:algorithms}.
Similar to the experiment in Sec. \ref{subsec:LQR_eval}, the federated learning algorithms use FedAVG to aggregate trained parameters.
In our method (APFL), we used layer-wise learning rate instead of parameter-wise due to computing efficiency.

\input{figure_latex/carlo_learning_curve}

\noindent \tu{Evaluation Results:}
We evaluate the test losses of the prediction models trained with the different algorithms.
Fig. \ref{fig:carlo_lc} shows how the losses have reduced during the federated learning.
In contrast to Standard FL, the algorithms involving personalization are going well,
in particular,  performs the lowest loss, and this is consistent with the results of the experiment in Sec. \ref{subsec:LQR_eval}.

Additionally, using the second dataset generated from the controllers with the prediction model, we evaluate how safe and efficiently the cars are able to swap lanes.
Fig. \ref{fig:carlo_boxplot} is a box plot showing the distributions of the elapsed time until starting lane change, distance between the cars at the time of starting lane change, and the mean cost for each session.
According to these box plots, the robot car controlled with a APFL model can start to change a lane quickly with safe distance to the human car.

\input{figure_latex/carlo_boxplot.tex}

\subsection{Lane change with CARLA simulator}
\label{subsec:lane_change}

%\input{figure_latex/lane_change.tex}

\begin{comment}
\begin{enumerate}
    \item explain why CARLA is better than CARLO (e.g. it is a photo-realistic simulator)
    \item discuss why the CARLA example is more sophisticated because you have another robot much in advance of it [green car]
    \item describe how we set up experiments: cost function, robot vehicle cost function, and how many users/trials we gathered data for
    \item describe the CVAE model architecture and cost function for MPC
    \item only describe boxplot gains since we already showed the learning curve in the previous figures
\end{enumerate}
\end{comment}

We added one more experiment to make sure the effectiveness for various practical driving scenarios.
There are two major changes from the previous experiment of the lane swapping scenario.
First, we test our method through a new scenario shown on the right side of Fig. \ref{fig:traffic_scenarios}.
This scenario is more sophisticated because criterion of human driver becomes more complicated thanks to adding the gray car.
Another thing is that we change the simulator to CARLA \cite{Dosovitskiy17}, which has a realistic simulation engine in terms of not only visualization but computation of physical dynamics.
These changes enable us to verify our method in a more sophisticated system environment.

\noindent \tu{Experimental Setup:}
Basically, we define the settings of this experiment based on the lane swapping case in \ref{subsec:lane_swapping}.
The system and control definition is the same except adding the state of the gray car.
%(Value ranges of the control items are re-defined according to the CARLA's specification.)
The architecture of the prediction model is exactly the same as the one in \ref{subsec:lane_swapping}, shown in Fig. \ref{fig:cvae_arch}.
The robot controller is also the same except it does not switch to the second phase where the robot is going to change a lane because robot cars do not change lanes in the scenario.
Additionally, we set a lower limit $C_{low}$ on the cost function to prevent the robot cars from unnecessarily increasing the distance to the human car after the both cars have safe and sufficient distance.
Therefore, the new cost function $J^\prime_t$ is denoted by $\max (C_{low}, J_t)$.

Unlike the lane swapping case, we use a programmed controller for human cars to test on uniformly diverse driving styles including extreme ones.
This controller is also a two-phase controller, but control inputs are decided according to the target velocity in the first phase.
The target velocity can be taken as high $v_{high}$ or low $v_{low}$, and is simply decided by the current state and driving preference only at every time step as following;
\begin{small}
\begin{align*}
v^{target}_t = \left\{
\begin{array}{ll}
v_{high} & \text{if}\;\; \gamma D_{rel} \geq 0 \;\land\; p^{hy}_{t} - p^{gy}_{t} \geq D_{safe}\\
v_{low} & \text{otherwise}
\end{array}
\right.
\end{align*}
\end{small}
$\gamma$ is a parameter representing the degree of preference for overtaking robot cars.
The grater $\gamma$ means a more aggressive driving style preferring overtaking.
$D_{rel}$ is a relative state based on the positions and velocities denoted by $(p^{hy}_{t} - p^{ry}_{t}) + (v^{hy}_{t} - v^{ry}_{t})$,
and $p^{gy}_t$ and $D_{safe}$ are a longitudinal position of the gray car and a safe distance constant, respectively.
The specific value of each target velocity is set depending on relative velocity to a robot car running alongside.
Once the target velocity is determined, the controller computes control inputs with the PID controller on CARLA.
We prepare 5 kinds of driving styles whose $\gamma$ parameters are $[-1.0,-0.5,0,0.5,1.0]$.
These driving styles include somewhat extreme ones.
For instance, a human car with $\gamma = 1.0$ sometimes tries to pass the robot car even when the current relative position to the robot car are negative.
That is how we ensure diversity of driving styles in this experiment.

We collected the dataset with the same way as the previous case.
We prepared 54 initial states where relative position and velocity is uniformly distributed.
We trained four types of the prediction models except Local shown in Tab. \ref{tab:algorithms} with the same hyper parameters as the previous case.
Finally, we evaluate 9 of 54 cases, which need the robot cars to change their behavior depending on human's driving styles, in performance of each controllers incorporating the prediction models trained with different ways.

\begin{table}[t]
\caption{\small{\textbf{Prediction loss for each prediction model}:
All values are losses on the test data after training has converged.
}}
\label{tab:lane_change_loss}
\centering
\begin{tabular}{c|c|c|c|c}
    \hline
    Algorithm & Cloud & SFL & SPFL & APFL\textbf{(Ours)} \\ \hline
    \hline
    Loss & 0.01643 & 0.01760 & 0.01600 & \textbf{0.01160} \\ \hline
\end{tabular}
\end{table}

\noindent \tu{Evaluation Results:}
Using the same metrics as the lane swapping case in Sec. \ref{subsec:lane_swapping}, we evaluate the test loss of the prediction model and the controllers' performance in terms of how safe and efficiently the cars are able to change a lane.
The prediction losses for each model, which are shown in Tab. \ref{tab:lane_change_loss}, have the same trend as in the previous scenario of lane swapping.
Regarding actual controllers' performance of traffic, as Fig. \ref{fig:carla_boxplot} illustrates, APFL provides the lowest cost while maintaining a safe distance from other cars.

\input{figure_latex/carla_boxplot.tex}

